Gen-T: Table Reclamation in Data Lakes

We introduce the problem of Table Reclamation. Given a Source Table and a large table repository, reclamation finds a set of tables that, when integrated, reproduce the source table as closely as possible. Unlike query discovery problems like Query-by-Example or by-Target, Table Reclamation focuses on reclaiming the data in the Source Table as fully as possible using real tables that may be incomplete or inconsistent. To do this, we define a new measure of table similarity, called error-aware instance similarity, to measure how close a reclaimed table is to a Source Table, a measure grounded in instance similarity used in data exchange. Our search covers not only SELECT-PROJECT- JOIN queries, but integration queries with unions, outerjoins, and the unary operators subsumption and complementation that have been shown to be important in data integration and fusion. Using reclamation, a data scientist can understand if any tables in a repository can be used to exactly reclaim a tuple in the Source. If not, one can understand if this is due to differences in values or to incompleteness in the data. Our solution, Gen-T, performs table discovery to retrieve a set of candidate tables from the table repository, filters these down to a set of originating tables, then integrates these tables to reclaim the Source as closely as possible. We show that our solution, while approximate, is accurate, efficient and scalable in the size of the table repository with experiments on real data lakes containing up to 15K tables, where the average number of tuples varies from small (web tables) to extremely large (open data tables) up to 1M tuples.

==> src/cover.tex <==
\newcommand{\reminder}[1]{{\mbox{$<==$}} [[[ { \bf #1 } ]]] {\mbox{$==>$}}}
\newcommand{\response}{\smallskip\noindent\normalfont\textbf{\textcolor{blue}{Response: }}}

\begin{center}
	\textbf{Response by Authors 936}\\
\end{center}

% \skip

\noindent 
Thank you for your thoughtful reviews and comments. We have revised the paper according to the reviewers' comments (changes are color-coded in \revision{blue}). 

% We understand that o
Our original submission did not explicitly state that our code is available. However, the code, all baselines (including our newly-added baselines Ver and ChatGPT), example experiment outputs and benchmark samples %for \name 
are all publicly available %on our GitHub repository
~\cite{gen-t_repo}: \url{https://github.com/northeastern-datalab/gen-t}

\section*{Baseline Query-by-Example Approaches}
{\it \noindent {\bf Meta Reviewer}: Justify the difference of this paper from Query-by-Example approaches.
}
%\\
({\it \noindent {\bf R2O1}: ``The authors claim that their work is different than Query-by-Example approaches. However, this is not well justified. That is, the target table can be the example we try to re- generate. Existing approaches already handle that: Ver~\cite{Gong2023Ver}, DICE~\cite{DBLP:journals/pvldb/RezigBFPVGS21}, and Dataset-on-Demand~\cite{DBLP:journals/corr/abs-1911-11876} to cite a few. The only difference is that the authors are covering a bigger set of queries. Also, unlike what the authors claim, those prior works also do not assume they know the subset of tables that can be used to re-construct the target view.'')
% \begin{itemize}
%     \item Dataset-On-Demand~\cite{DBLP:journals/corr/abs-1911-11876} 
%     \item Ver~\cite{Gong2023Ver}
% \end{itemize}
}

\response
We agree that prior works on Query-By-Example such as Ver~\cite{Gong2023Ver}, DICE~\cite{DBLP:journals/pvldb/RezigBFPVGS21}, and Dataset-on-Demand~\cite{DBLP:journals/corr/abs-1911-11876} can be adapted to solve the problem of table reclamation. As the reviewer mentions, some QBE approaches do not assume that they know the subset of tables that were originally used to generate the query view, and aim to discover views that contain the query view. However, the goal of QBE problem is different from the table reclamation problem. QBE aims to ``help non-expert users complete a partially fulfilled query view''~\cite{DBLP:journals/corr/abs-1911-11876}. Table Reclamation aims to reproduce the source table \emph{as closely as possible}, with no assumption that the source table is only partial. Unlike QBE systems, \name can reproduce large source tables that consist of many tuples (we experiment with source tables containing up to 22 columns and 1K rows (Section~\ref{subsec:exp_setup})), rather than small source tables that QBE systems experiment with (e.g., Ver~\cite{Gong2023Ver} uses queries that are tables of 2 columns and 3 rows). Finally, as the reviewer points out, compared to prior work on Query-by-Example, we do consider a larger set of queries that could have been used to originally generate the Source Table, namely Select-Project-Join-Union queries. We have added a clarification in the second paragraph in ``Finding Origins of Tables'' (Section~\ref{sec:related}).

% \smallskip

{\it \noindent {\bf Meta Reviewer}: Compare Gen-T with more baselines, e.g., Ver (a query-by-example system that supports PJ queries). ({\bf R2O3})
}
% \\
% {\it \noindent {\bf R2O3}: The authors did not include state-of-the-art approaches as baselines to evaluate their work. For instance, it would be informative to see how Gen-T compares to Ver (a query- by-example system that supports PJ queries).
% }

\response
We have added a comparison with Ver~\cite{Gong2023Ver}
%rjm on our smallest benchmark, \tpchSmallBench, 
in Table~\ref{tab:small-effectiveness} (Section~\ref{sec:experiments}). For each source table, we give Ver a collection of
%\rjm{is it clear what index means here?}\grace{changed} 
originating tables. When we query with our source tables, we find that Ver cannot scale to our full source table sizes.  % of $\sim$9 columns and 27 rows. 
In the experiments reported in~\cite{Gong2023Ver}, 
%\rjm{if you really mean mainly - state other queries they use}  
queries with tables that have 2 columns and 3 rows are reported.  To accommodate these limitations, we ran Ver with only two columns from our Source Tables and aggregated the results in order to evaluate the entire source table. Due to the scalability constraint of Ver, we only report results on our smallest benchmark \tpchSmallBench (source table size of $\sim$9 columns and 27 rows), as Ver did not finish on other benchmarks within 24 hours. In our experimental results, we find the results are comparable with \aPip~\cite{DBLP:journals/pvldb/YangHC21}, a Query-By-Target approach that we also use as a baseline. Output tables from Ver contain many tuples from the source table (high Recall), but because Ver does not perform Selection on tuples, the output tables also contain many extraneous tuples (low Precision). This output makes sense in the context of Query-by-Example, whose goal is to provide additional tuples in addition to those in the source table. However in our problem, we only want to reproduce the tuples from a source table. 

The demo paper DICE~\cite{DBLP:journals/pvldb/RezigBFPVGS21} and Dataset-on-Demand~\cite{DBLP:journals/corr/abs-1911-11876} do not openly provide their code. Considering the limited revision time ($<$ 3 weeks), we were unable to recreate their code and use them as baselines. 
%\rjm{Does Ver compare to DICE or Dataset-on-Demand?}\grace{No :(. DICE cites DoD, but doesn't compare}
However, we would expect DICE and Dataset-on-Demand to return similar results as Ver, since they all have the same problem setting. 
Dataset-on-Demand~\cite{DBLP:journals/corr/abs-1911-11876} has not yet been peer-reviewed, but has a similar architecture as Ver. Given a query view, Dataset-on-Demand discovers and combines datasets to produce a view that contains the query view, while being space and time efficient. Thus, running Dataset-on-Demand for our problem of table reclamation would likely produce similar results as Ver. 
DICE~\cite{DBLP:journals/pvldb/RezigBFPVGS21} also only considers a few example records provided by the user,
%\rjm{this is very good, but if you can make specific that is even better -- e.g. DICE also on considers query tables with up to C columns and R rows in their experiments.} 
then aims to return more records. Thus, we would also expect Dice to return similar results as Ver.
% \rjm{should we explain what we would expect to get?  e.g., Dataset-on-Demand has not yet been peer-reviewed but is similar to Ver in the following way... so we would expect similar results.  DICE also only considers queries up to....}
% \grace{added. In DICE (and in their main paper), they don't specify size of queries they experiment with.}



% \smallskip

{\it \noindent {\bf Meta Reviewer}: Compare Gen-T with LLMs. ({\bf R3O1})
}
% \\
% {\it \noindent {\bf R3O1}: A comparison with a method based on using LLMs should be added
% }

\response
We have added a comparison with OpenAI's LLM ChatGPT3.5~\cite{chatgpt}. Due to scalability constraints,
%rjm:  I think the  constraints are different in nature, right?
%similar to above, 
we could only run this baseline on \tpchSmallBench (see new Table~\ref{tab:small-effectiveness} in Section~\ref{sec:experiments}). Specifically, in the case of LLMs, the input token limit constraints the size of both the provided source tables and the data lake or integrating tables.

In our prompt, we define the table reclamation problem and provide a Source Table and its 
%integrating set (made up of its
set of originating tables. %Considering the token limit of ChatGPT3.5, we are unable to input the entire data lake. 
ChatGPT then returns a tabular result of integrating the provided integrating set with the goal of reproducing (reclaiming) the source table. As shown in Table~\ref{tab:small-effectiveness}, ChatGPT is only able to reproduce some tuples from the source table, while returning many extraneous tuples. The high divergence scores indicate that ChatGPT returns many non-null values that contradict values from the Source Table. 

In future work, we can make use of larger models (e.g., GPT4) and learn to tokenize large data lakes to accommodate the token limit.
However, we expect there will still be benefits from our search and pruning approach. From a data lake, we need to discover and integrate tables that are needed to reproduce the source table, while keeping the integration space small. Even if we prompt LLMs with a large data lake, there is no guarantee that they will extract a small and complete set of tables as originating tables. When integrating the tables in a targeted manner, there is also no guarantee that these models will not hallucinate (i.e., invent tuples or values not in the data lake).
%and only draw from tuples from the originating tables. 
Thus, an effective search method is needed when we have a large data lake.
%and a proper pruning technique is needed to maintain space and time efficiency.
% \rjm{Should we add:  but we expect there will still be benefits from our search approach -- or something more precise?  }
% \grace{added}

\section*{Assumption}
{\it \noindent {\bf Meta Reviewer}:  Revise or justify well the strong assumption of this paper. 
}
% \\
% {\it \noindent {\bf R1D3}:  Even though the author did not make assumptions about including keys in the tables from the data lake, their efficient integration is heavily dependent on that property.
% }
% \\
({\it \noindent {\bf R2O4}:  ``The authors claim they can support a wide range of queries, however, strong assumptions are being made, ``In our solution, we assume the Source Table has a key, and thus align tuples by matching using equality on the key". This makes finding joins much easier for example. In data lakes, it is often the case that tables have no key columns or multiple ones.'' + {\bf R1D3})
}

\response
We assume that Source Tables have keys, which makes instance comparison fast. We do not assume that data lake tables have keys. To find data lake tables that can reproduce the Source Table, we focus on finding tables that have the same column values as the Source Table, then perform integration.  Because the data lake tables often have no keys, they may produce multiple copies of source tuples and our method handles this.  
%We understand that our assumption that Source Tables contain keys is restricting.  
At the time of submission there were no fast instance comparison algorithms for the general case (instance comparison requires homomorphisms checks which are exponential), but fast comparison is possible if one of the two tables being compared has a key (this is our setting where Source Table has a key and integrated data lake tables do not).  Fast approximate algorithms for the general case is an interesting research problem on its own that has only been addressed in an upcoming EDBT24 paper~\cite{Glavic2024}.  In future work, we plan to use this approximate algorithm to address the general case of Source Tables without keys (we have added this point in future work Section~\ref{sec:conclusion}).  Understanding if this approximate algorithm is fast enough and accurate enough to be used for reclamation is beyond the scope of this paper.
We have elaborated on our key assumption in the second paragraph in Section~\ref{sec:overview} and in the first paragraph in Section~\ref{subsec:tuple_alignment}.
%, and we will relax this assumption in future work by using a newly proposed method for approximate instance comparison~\cite{Glavic2024}. \grace{@Renee, can you add more about approximate instance comparison?}


\section*{Schema matching and Record alignment}
{\it \noindent {\bf Meta Reviewer}: Justify the over-simplication of the paper. For example, why can you omit the issues of schema matching and record alignment. ({\bf R1O2})
}
% \\
% {\it \noindent {\bf R1O2}: The paper oversimplified big problems such as schema matching and record alignment, which is known to be a challenging task regardless of the tremendous amount of literature in the area. It is understandable that the paper is not about schema matching (mapping) but this subtask is critical for the success of such system.
% }

\response
We agree that schema matching and record alignment are challenging tasks, especially in the context of data lakes. In our setting, we assume that the Source Tables have key attributes (see clarification above), and thus align records (tuples) based on the key values from the Source Tables. We discuss the alignment of tuples using the key in Section~\ref{subsec:tuple_alignment}. We implicitly perform schema matching by finding columns from data lake tables that have high value overlap with columns from a Source Table, and rename the data lake tables' columns with the Source Table's column name. 
We have elaborated on this point in Section~\ref{subsec:candidate_table_retrieval}. We have also updated the related work (``Table Integration'', Section~\ref{sec:related}) accordingly. 
%rjm:  I don't think you need to repeat this
%In future work, this key assumption is to be relaxed by using...~\cite{Glavic2024}. \grace{Complete}

% \smallskip

\section*{Similarity Score}
{\it \noindent {\bf Meta Reviewer}: Consider more semantical similarity scores. ({\bf R2O2})
}
% \\
% {\it \noindent {\bf R2O2}: The instance similarity score only takes into account the syntactic similarity score between instances. This is a limiting factor since in many cases values can be semantically the same but syntactically different.
% }

\response
While some recent Query-By-Example methods~\cite{Gong2023Ver,DBLP:journals/corr/abs-1911-11876} consider semantic similarity between attributes (e.g., home addresses vs. work addresses), they rely on a human-in-the-loop to disambiguate the attributes. In our current problem setting, \name aims to reproduce all values from the Source Table, as is. To disambiguate instances, we currently only consider syntactic similarity between instances in the data lake and those in the Source Table. We believe that if the reproduced Source Table contains the same values as those in the Source Table, then it must share the same semantics as the Source Table. We have added this clarification in Section~\ref{subsec:tuple_alignment}.
While Ver~\cite{Gong2023Ver} does consider semantic matching of values, recall it does so on query tables with at most 2 columns and 3 rows.  Making semantic matching of values scale to the query sizes we consider, and doing so meaningfully when the objective is table reclamation rather than QBE, is an interesting topic that we now mention in future work Section~\ref{sec:conclusion}.
%It is important to note that we currently assume that all values in a source table directly descended from values in a data lake, with no alterations made to the values. We understand that this assumption is not practical, especially if we consider adversarial attacks on the original integration process. In future work, we will relax this assumption and explore semantic similarity of values that may have changed over the original integration process. We have added this note in Section~\ref{sec:conclusion}.

% \smallskip

\section*{Presentation}
{\it \noindent {\bf Meta Reviewer}: Reduce the discussion in multiple places to make room for adding more important details and increase the self explanation of the paper. ({\bf R1O1})
}
% \\
% {\it \noindent {\bf R1O1}: The discussion in multiple places took more space than it supposed to, which was on the expense of omitting important information in the paper and referring the reader to the technical report. It would be great to reduce those sections to make room for adding more important details and increase the self explanation of the paper. For example, you don't have to remind the reader about what is going to be discussed in each subsection after giving the big picture of the section.
% }

\response
We %have 
reduced the discussion in multiple places across the paper to make room for the above-mentioned additions. 
% \todo{this requires surgery on the paper} \roee{As this is a general item, I think our response can be general as well. This will be reflected in the triming that we will perform. If we end up removing a major part, we can add a spesific note here as well.}

% \smallskip
\section*{Other Comments}

{\it \noindent {\bf R1D2}: Matrix Traversal Discussion 
% The discussion about the matrix traversal can be more concise to increase readability. Need to explain why $m_r[j] = max(t_1[j], t_2[j])$. Even though it was explained later, it is important to explain it where it was mentioned first so the reader can follow the discussion better.
}

\response
We have made this discussion more concise and added the following clarification to Section~\ref{subsec:matrix_traversal}. Suppose we have matrices $m_1, m_2$. At row index $i$, we have tuples $t_1, t_2$, from $m_1, m_2$, respectively. After combining $m_1, m_2$, the resulting matrix has tuple $m_r$ at row index $i$.
At column $j$, $m_r[j] = max(t_1[j], t_2[j])$. This is equivalent to taking the logical {\tt OR} of the values at index ($i$, $j$) in the two matrices $m_1, m_2$. If $t_1[j]$ and $t_2[j]$ are 1, then $m_r[j]$ is 1. If $t_1[j]$ is 1 and $t_2[j]$ is 0, or vice versa, then $m_r[j]$ is 1. If both $t_1[j]$ and $t_2[j]$ are 0, then $m_r[j]$ is 0. 
%We have added this clarification to Section~\ref{subsec:matrix_traversal}.

\smallskip
% \section*{Diversifying Tables}
{\it \noindent {\bf R1D1}: Diversifying Tables Details
% The authors mentioned about diversifying the tables that can be used in the reconstruction process. The discussion is a little high level and no formula to rank the tables according to their relevance and diversity. The complementation operator can be used to discard duplicate tables but what would happen if tables overlap in few attributes only?
}

\response
% After we retrieve a set of candidate tables from a data lake, for which we use Starmie~\cite{starmie22} to retrieve the top-$k$ unionable tables from a data lake in our experiments, we diversify the candidate tables.
After we retrieve a set of top-$k$ candidate tables from a data lake, we diversify them to ensure that each candidate table not only has high set overlap with the Source Table, but also is diverse from other candidate tables. As we mention in Section~\ref{subsec:candidate_table_retrieval}, this is especially important in public data lakes, which tend to have multiple versions of the same tables~\cite{DBLP:journals/pvldb/ShragaM23,koch2023duplicate} and a large percentage of duplicate column sets~\cite{DBLP:conf/sigmod/ZhuDNM19}. Specifically, if a candidate table is a duplicate or contained in another, then, using diversification, it can be pushed out of the top-$k$ ranking to avoid using the same data twice. We incorporate diversity into our set overlap score by measuring the set overlap of a candidate table, $T_i$, with the Source Table, $S$, versus its overlap with other candidate tables, $T_{i-1}$. We have updated the discussion and added 
%the following formula 
Formula~\ref{eq:diverseScore} to Section~\ref{subsec:candidate_table_retrieval}. 

%rjm  I don't think you need this in cover letter
%(Formula~\ref{eq:diverseScore}).
%$$
%    \text{diverseOverlapScore} = \frac{|T_i \cap S|}{|S|} - \frac{|T_i \cap T_{i-1}|}{|T_i|} 
%$$
%
%If a candidate table overlaps with another on only a few attributes and has a high set overlap with the Source Table, it has a high score and remains as a candidate table. 
% \grace{@Roee, please confirm}


==> src/tablePreparation.tex <==
%rjm:  I suggest removing this

\subsection{Preparing Originating Tables}\label{subsec:prep_tables}
% organizing or understanding candidate tables:
% 1. how you align columns of the candidate tables with the Source Table
% 2. how you finding tables that contain the Source Table key,  
% 3. how you find tables that share all attributes and can be unioned
% 4. how you determine tables that contain Source Table columns but not the key that can still be joined with another or many (key containing) candidate tables.
% describe a FK finding algorithm.
%rjm resolved
%\roee{I would also add forward references when ever we mention we will do something, e.g., in the discovery phase. Also, I don't think we have to say here the originating tables come from a discovery phase (especially since we have experiments in which we are given the originating tables. I would change the wording a bit to say, for example, "Given a set of originating tables, which can be generated using our Table Discovery phase (Section~\ref{sec:discovery}), ..."}
Given a set of originating tables, which may be found using our Table Discovery phase (Figure~\ref{fig:pipeline}), we first prepare them for Table Integration. Before 
%rjm integrating this set of originating tables, 
integration, we align the columns and tuples of each originating table to the Source Table, and organize the set of tables so that Table Integration can effectively produce a possible reclaimed table in an efficient manner.

First, we align the columns in each originating table to the Source Table's columns. To do so, for every column in an originating table that contains many values from a column in the Source Table (found in the Table Discovery phase), we rename the column with the corresponding Source Table's column's name. Then, we remove any extraneous columns whose values are not found in the Source Table.  \renee{hmm, this is vague, what if a column matches more than one source column?  What is definition of extraneous - no overlapping values at all?  so if there is one overlapping value the column is aligned with the one or more columns containing that value?  Can we describe this using attribute matching terminology?}
%We assume that an alignment between the originating tables and the source table (attribute-match, denoted Σ) is given and that tuples are aligned via the source key.

Next, we align the tuples in each originating table to the Source Table's tuples. 
Recall that we assume the tables have primary and/or foreign keys. 
% From the previous Table Discovery phase, we find a set of originating tables such that for every data lake table that does not have the Source Table's primary key, we join it with another data lake table that does. This way, all originating tables have the Source Table's primary key, and we can use key values to identify and align tuples between each originating table and the Source Table. 
To make use of keys, there are techniques in place to discover candidate keys~\cite{DBLP:conf/icde/AbedjanQN14,DBLP:journals/pvldb/HeiseQAJN13} and foreign keys that automatically discover primary key / foreign key relationships in tables~\cite{Buranosky2018FDToolAP} or infer minimal keys from mined functional dependencies~\cite{DBLP:conf/webdb/RostinABNL09}. 

Once all originating tables have their columns and tuples aligned with the Source Table, we organize them in relation to each other before integrating them. We first see if any schemas in the set of originating tables exactly align. If so, we can directly union their tables and reduce the search space in table integration. To determine the alignments of schemas, we iterate through each originating table and find other table(s) that share the exact same schema. Note that at this point, all originating tables only contain columns from $S$, such that all of their column names align with $S$'s column names, and thus with each other.

\renee{hmm, what does "next to each other" mean?  We have a set of originating tables. what is the significance of order?}
Lastly, we arrange the set of originating tables so that tables next to each other can be integrated on common columns. When performing table integration, we ingest each originating table in order. Thus, arranging this set of tables is crucial in making sure that there are common columns between a pair of tables in every integration step, especially since each table may only contain some of the Source Table's columns. In preparing for integration, we order the tables first by the number of Source Table's values found in each table, then arrange the tables so that neighboring tables have some columns in common, preferably with a primary key / foreign key relationship. This way, when we integrate the ordered list of originating tables, the integration result can have less noisy and extraneous tuples, compared to the Source Table. 


